Enhanced word embeddings using multi-semantic representation through lexical chains

The relationship between words in a sentence often tells us more about the underlying semantic content of a document than its actual words, individually. In this work, we propose two novel algorithms, called Flexible Lexical Chain II and Fixed Lexical Chain II. These algorithms combine the semantic relations derived from lexical chains, prior knowledge from lexical databases, and the robustness of the distributional hypothesis in word embeddings as building blocks forming a single system. In short, our approach has three main contributions: (i) a set of techniques that fully integrate word embeddings and lexical chains; (ii) a more robust semantic representation that considers the latent relation between words in a document; and (iii) lightweight word embeddings models that can be extended to any natural language task. We intend to assess the knowledge of pre-trained models to evaluate their robustness in the document classification task. The proposed techniques are tested against seven word embeddings algorithms using five different machine learning classifiers over six scenarios in the document classification task. Our results show the integration between lexical chains and word embeddings representations sustain state-of-the-art results, even against more complex systems.

==> tables/ex_build_chains.tex <==
\begin{table}[htb]
 \centering
  \caption{Lexical chains construction.}
  \label{tab:chains_construction}
 \resizebox{1.0\textwidth}{!}{
   \begin{tabular}{lc} \toprule
      Lexical Chain Type   & Lexical Chain \\ \midrule
      \multirow{2}{*}{A - FLLC II}  &\{A1:\{beet.n.02, carrot.n.03, potato.n.01\}, A2:\{grandma.n.01, grandfather.n.01\}, \\ & A3:\{favorite.n.01\}, A4:\{dish.n.02, lunch.n.01\}\}   \\ \hline
      \multirow{2}{*}{B - FXLC II}  &\{B1:\{beet.n.02, carrot.n.03, potato.n.01\}, B2:\{grandma.n.01, grandfather.n.01, \\ & favorite.n.01\}, B3:\{dish.n.02, lunch.n.01\}\}   \\
      \bottomrule
    \end{tabular}
  }
\end{table}

==> tables/ex_chains_avg_vectors.tex <==
\begin{table}[htb]
  \caption{Vector average for lexical chains \emph{centroids}.}
  \centering
  \label{tab:chains_avg}
  \resizebox{0.88\textwidth}{!}{
   \begin{tabular}{lcrrrrr} \toprule
     Lexical Chain Type &Centroid   & Dim-01     & Dim-02     & Dim-03   & Dim-04     & Dim-05 \\ \midrule
       \multirow{4}{*}{A - FLLC II}  &A1	&-0.091	&0.270	&0.520	&-0.135	&0.388\\
        &A2	&0.062	&-0.163	&0.240	&0.532	&0.489\\
        &A3	&0.121	&0.581	&-0.603	&0.148	&0.046\\
        &A4	&-0.104	&0.101	&0.283	&0.509	&0.519\\ \midrule
        \multirow{3}{*}{B - FXLC II} &B1	&-0.091	&0.270	&0.520	&-0.135	&0.388\\
        &B2	&0.082	&0.085	&-0.041	&0.404	&0.341\\
        &B3	&-0.104	&0.101	&0.283	&0.509	&0.519\\ 
      \bottomrule
    \end{tabular}
   }
\end{table}

==> tables/ex_chains_finished.tex <==
\begin{table}[htb]
 \centering
  \caption{Final chains for FLLC II and FXLC II algorithms.}
  \label{tab:chains_finished}
 \resizebox{0.85\textwidth}{!}{
   \begin{tabular}{lc} \toprule
      Lexical Chain Type   & Lexical Chain  \\ \midrule
      FLLC II  &\{potato.n.01, grandma.n.01, favorite.n.01, lunch.n.01\}   \\
      FXLC II  &\{potato.n.01, grandfather.n.01, lunch.n.01\}   \\
      \bottomrule
    \end{tabular}
  }
\end{table}

==> tables/ex_chains_sentence.tex <==
\begin{table}[htb]
 \centering
  \caption{Sentence example transformation from words into synset.}
  \label{tab:sentence_synset_steps}
 \resizebox{1.0\textwidth}{!}{
   \begin{tabular}{lL{12cm}} \toprule
      Type                                      & Sentence                                                                                          \\ \midrule
      \multirow{2}{*}{Original Sentence}        & Beets, carrots, and potatoes are grandma and grandpa \textquotesingle s favorite dish for lunch!  \\ \cmidrule{2-2}
      Pre-Processed Sentence                    & \{beets, carrots, potatoes, grandma, grandpa, favorite, dish, lunch\}                             \\\cmidrule{2-2}
      \multirow{3}{*}{Synset Sentence}          &\{Synset(`beet.n.02'), Synset(`carrot.n.03'), Synset(`potato.n.01'), Synset(`grandma.n.01'),  Synset(`grandfather.n.01'), Synset(`favorite.n.01'), Synset(`dish.n.02'), Synset(`lunch.n.01')\}   \\\cmidrule{2-2}
      \multirow{2}{*}{Filtered Synset Sentence} &\{beet.n.02, carrot.n.03, potato.n.01, grandma.n.01, grandfather.n.01, favorite.n.01, dish.n.02, lunch.n.01\}   \\
      \bottomrule
    \end{tabular}
  }
\end{table}

%multirow{2}{*}{Filtered Synset Sentence}  &\{beet.n.02, carrot.n.03, potato.n.01, grandma.n.01, \\ & grandfather.n.01, favorite.n.01, dish.n.02, lunch.n.01\}   \\

==> tables/ex_chains_synsets.tex <==
\begin{table}[htb]
  \caption{Sample of related synsets extracted from WordNet.}
  \label{tab:related_synset}
 \resizebox{\textwidth}{!}{
   \begin{tabular}{llll} \toprule
    Main Synsets        & Related Synset 01     & Related Synset 02     & Related Synset 03     \\ \midrule
    beet.n.02           & root\_vegetable.n.01  & sugar\_beet.n.02      & beetroot.n.01         \\
    carrot.n.03         & carrot.n.02           & root\_vegetable.n.01  &  -                    \\
    potato.n.01         & baked\_potato.n.01    & french\_fries.n.01    & root\_vegetable.n.01  \\
    grandma.n.01        & grandparent.n.01      & nan.n.01              &  -                    \\
    grandfather.n.01    & grandparent.n.01      & -                     &  -                    \\
    favorite.n.01       & choice.n.01           & -                     &  -                    \\
    dish.n.02           & nutriment.n.01        & meal.n.01             &  ingredient.n.03      \\
    lunch.n.01          & meal.n.01             & business\_lunch.n.01  & -                     \\
    \bottomrule
    \end{tabular}
  }
\end{table}


==> tables/ex_cosinesim_chains.tex <==
\begin{table}[htb]
\caption{Cosine similarity between lexical chains and their centroids.}
  \label{tab:chains_sim}
 \resizebox{\textwidth}{!}{
\begin{tabular}{lcrlcr} \toprule
    \multicolumn{3}{c}{FLLC II}           & \multicolumn{3}{c}{FXLC II}            \\ \hline{|}
    Synset           & Centroid & CosineSim & Synset           & Centroid & CosineSim  \\ \midrule
    beet.n.02        & A1     & 0.264     & beet.n.02        & B1     & 0.264      \\
    carrot.n.03      & A1     & 0.509     & carrot.n.03      & B1     & 0.509      \\
    potato.n.01      & A1     & \textbf{0.578}     & potato.n.01      & B1     & \textbf{0.578}      \\
    grandma.n.01     & A2     & \textbf{0.815}     & grandma.n.01     & B2     & 0.420      \\
    grandfather.n.01 & A2     & 0.572     & grandfather.n.01 & B2     & \textbf{0.882}      \\
    favorite.n.01    & A3     & \textbf{1.000}     & favorite.n.01    & B2     & 0.341      \\
    dish.n.02        & A4     & 0.365     & dish.n.02        & B3     & 0.365      \\
    lunch.n.01       & A4     & \textbf{0.746}     & lunch.n.01       & B3     & \textbf{0.746}      \\    
    \bottomrule
    \end{tabular}
    }
\end{table}

==> tables/ex_tsm_vectors.tex <==
\begin{table}[htb]
  \caption{Fictional pre-trained synset embeddings model.}
  \centering
  \label{tab:synset_vectors}
%  \resizebox{\textwidth}{!}{
   \begin{tabular}{lrrrrr} \toprule
    Synsets             & Dim-01    & Dim-02    & Dim-03    & Dim-04    & Dim-05    \\ \midrule
    beet.n.02           & 0.926	    & 0.620	    & -0.278	& -0.380	& 0.717     \\
    carrot.n.03	        & -0.525	& 0.361	    & 0.839	    & -0.989	& -0.420    \\
    potato.n.01	        & -0.675	& -0.172	& 1.000	    & 0.964	    & 0.868     \\
    grandma.n.01	    & 0.159	    & -0.795	& 0.663	    & 0.405	    & 0.617     \\
    grandfather.n.01	& -0.035	& 0.469	    & -0.183	& 0.659	    & 0.361     \\
    favorite.n.01	    & 0.121	    & 0.581	    & -0.603	& 0.148	    & 0.046     \\
    dish.n.02	        & 0.667	    & -0.257	& -0.379	& 0.300	    & 0.723     \\
    lunch.n.01	        & -0.874	& 0.458	    & 0.945	    & 0.717	    & 0.314     \\
      \bottomrule
    \end{tabular}
%   }
\end{table}

==> tables/gridsearch_configuration.tex <==
\begin{table}[htb]
\centering
\caption{Grid search configuration.}
\label{tab:gridsearch}
\resizebox{0.92\textwidth}{!}{
  \begin{tabular}{llr}
  \toprule
    Classifier                                                                        & Parameter             & Range                                       \\\midrule
    k-NN                                                                              & neighbors             & 1, 5, 15, 25 \ldots{} 95                    \\\cmidrule(lr){2-3}
    \multirow{4}{*}{\begin{minipage}{0.7in}Logistic\\ Regression\end{minipage}}       & solver                & newton-cg, lbfgs, sag, saga                 \\
                                                                                      & maximum iteration     & 500, 1000, 1500                             \\
                                                                                      & multi-class           & ovr, multinomial                            \\
                                                                                      & tolerance             & 0.01, 0.001, 0.0001, 0.00001                \\\cmidrule(lr){2-3}
    \multirow{4}{*}{\begin{minipage}{0.5in}Support\\ Vector\\Machine\end{minipage}}   & kernel                & linear, radial bases function, polynomial   \\
                                                                                      & gamma                 &  0.01, 0.001, 0.0001, 0.0001                \\
                                                                                      & polynomial degree     & 1, 2, 3, 4, 5, 6, 7, 8, 9                   \\
                                                                                      & C                     & 1, 10, 100                                  \\\cmidrule(lr){2-3}
     \multirow{5}{*}{\begin{minipage}{0.5in}Random\\Forest\end{minipage}}             & number of estimators  & 100, 325, 550, 775, 1000                    \\
                                                                                      & maximum features      & auto, sqrt                                  \\
                                                                                      & maximum depth         & 10, 32, 77, 100, None                       \\
                                                                                      & minimum samples split & 2, 5, 10                                    \\
                                                                                      & minimum samples leaf  & 1, 2, 4                                     \\
    \bottomrule
  \end{tabular}
 } 
\end{table}

